Estimation of Spectral Biophysical Skin Properties from Captured RGB Albedo

We present a new method to reconstruct and manipulate the spectral properties of human skin from simple RGB albedo captures. To this end, we leverage Monte Carlo light simulation over an accurate biophysical human skin layering model parameterized by its most important components, thereby covering a plausible range of colors. The practical complexity of the model allows us to learn the inverse mapping from any albedo to its most probable associated skin properties. Our technique can faithfully reproduce any skin type, being expressive enough to automatically handle more challenging areas like the lips or imperfections in the face. Thanks to the smoothness of the skin parameters maps recovered, the albedo can be robustly edited through meaningful biophysical properties.

==> fig/teaser.tex <==
% A "teaser" figure, centered below the title and authors and above the body of the work.
\begin{teaserfigure}
  \centering
  %\includegraphics[draft, width=\linewidth]{fig/teaser.png}
  \includegraphics[width=\linewidth]{fig/teaser2.jpg}
  \caption{Our framework reconstructs, given a captured albedo, the main skin properties that lead to a particular diffuse reflectance. We leverage Monte Carlo simulations of light transport in small skin patches to create a space of biophysically plausible skin tones, coupled with an encoder-decoder model to finally build a bijective mapping from albedo to skin properties and vice versa. From left to right, renders of two manipulations on the haemoglobin concentration a) x0.125 haemoglobin b) x3 haemoglobin, c) render using the original albedo map, and renders of two manipulations on the melanin concentration d) x3 melanin e) x0.5 melanin. The model is generic to reconstruct any skin type, and robust to extreme edits or interpolations in the skin properties.}
  \label{fig:teaser}
\end{teaserfigure}

==> sec/conclusion.tex <==
\section{Conclusions}



\begin{acks}
%The authors would like to thank Dr. Yuhua Li for providing the MATLAB code of the \textit{BEPS} method.
%The authors would also like to thank the anonymous referees for their valuable comments and helpful suggestions. The work is supported by the \grantsponsor{GS501100001809}{National Natural Science Foundation of China}{https://doi.org/10.13039/501100001809} under Grant No.: ~\grantnum{GS501100001809}{61273304}
%21 and ~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young Scientists' Support Program}.
\end{acks}

==> sec/overview.tex <==
\section{Overview}

%CHERY: removed the (wrong) step on albedo spectral upsampling
%The process is composed of three steps. First, we upscale the input diffuse albedo from RGB to multi-band spectral using a recent approach~\cite{Mallett2019} (note that we could rely on other concurrent works~\cite{Jakob2019Spectral} to this end). Next, we infer

The process is composed of two steps. First, we infer the key parameters affecting skin appearance from a diffuse albedo capture. For this, we fit the albedo map to a high dimensional space of biophysical skin albedos, composed of a wide variety of spectral responses of 2D skin patches. The precomputation of skin tones generates a high dimensional tensor of all possible combinations of skin parameters. The details of our biophysical skin model are in Section \ref{sec:biophysical_model}. Once the skin properties are recovered, we can reconstruct identically the albedo, or manipulate the skin parameters in such latent space, creating new samples of human skin in a biophysically-based way. Section~\ref{sec:parameter_estimation} lays out the specifics of this inversion. Sections~\ref{sec:neural_estimation} and~\ref{sec:editing} show some skin parameters inference and manipulation over several skin types covering the Fitzpatrick scale~\cite{fitzpatrick1988validity}.


\endinput
\section{Overview}

%CHERY: removed the (wrong) step on albedo spectral upsampling
%The process is composed of three steps. First, we upscale the input diffuse albedo from RGB to multi-band spectral using a recent approach~\cite{Mallett2019} (note that we could rely on other concurrent works~\cite{Jakob2019Spectral} to this end). Next, we infer

The process is composed of two steps. First, we infer the key parameters affecting skin appearance. For this, we fit the albedo map to a high dimensional space of biophysical skin albedos, composed of a wide variety of spectral responses of 2D skin patches. The precomputation of skin tones generates a high dimensional tensor of all possible combinations of skin parameters, namely the skin structure and its chemical components, based on measurements from the optics and medical literature. The details of our biophysical skin model are in Section \ref{sec:biophysical_model}. Once the skin properties are recovered from the original albedo capture, we can reconstruct identically the albedo, or manipulate the skin parameters in such latent space, creating new samples of human skin in a biophysically-based way. Section~\ref{sec:parameter_estimation} lays out the specifics of this inversion, comparing an initial approach based on a large look-up tensor with our final neural parameter estimation, which outperforms in efficiency and editing quality its tabulated counterpart. Sections~\ref{sec:neural_estimation} and~\ref{sec:editing} show some skin parameters inference and manipulation over several skin types covering the Fitzpatrick scale~\cite{fitzpatrick1988validity}.

